Modeling and Performance Analysis of Full-Duplex Communications in Cache-Enabled D2D Networks

Cache-enabled Device-to-Device (D2D) communication is widely recognized as one of the key components of the emerging fifth generation (5G) cellular network architecture. However, conventional half-duplex (HD) transmission may not be sufficient to provide fast enough content delivery over D2D links in order to meet strict latency targets of emerging D2D applications. In-band full-duplex (FD), with its capability of allowing simultaneous transmission and reception, can improve spectral efficiency and reduce latency by providing more content delivery opportunities. In this paper, we consider a finite network of D2D nodes in which each node is endowed with FD capability. We first carefully list all possible operating modes for an arbitrary device using which we compute the number of devices that are actively transmitting at any given time. We then characterize network performance in terms of the success probability, which depends on the content availability, signal-to-interference ratio (SIR) distribution, as well as the operating mode of the D2D receiver. Our analysis concretely demonstrates that caching dictates the system performance in lower target SIR thresholds whereas interference dictates the performance at the higher target SIR thresholds.

==> ReferencesStyle.tex <==
@String { allerton        = {Proc., Allerton Conf. on Commun., Control, and Computing}}

@String { annor           = {Ann. Oper. Res.} }

@String { asilomar        = {Proc., IEEE Asilomar} }

@String { commletters     = {IEEE Commun. Letters} }

@String { commmag         = {IEEE Commun. Magazine} }

@String { commsnt         = {IEEE Commun. Surveys and Tutorials} }

@String { ctw             = {IEEE Commun. Theory Workshop} }

@String { elecletters     = {Electronics Letters} }

@String { ett             = {Trans. on Emerging Telecommunications Technologies} }

@String { globecom        = {Proc., IEEE Globecom} }

@String { globecomw       = {Proc., IEEE Globecom Workshops} }

@String { icassp          = {Proc., IEEE Intl. Conf. on Acoustics, Speech, and Sig. Proc. (ICASSP)} }

@String { icc             = {Proc., IEEE Intl. Conf. on Commun. (ICC)} }

@String { ieeetassp       = {IEEE Trans. on Acoustics, Speech, and Signal Processing} }

@String { infocom         = {Proc., IEEE INFOCOM} }

@String { isit            = {Proc., IEEE Intl. Symposium on Information Theory} }

@String { ita             = {Proc., Information Theory and its Applications (ITA)} }

@String { jsac            = {IEEE Journal on Sel. Areas in Commun.} }

@String { milcom          = {Proc., IEEE MILCOM} }

@String { mobicom         = {Proc., ACM MobiCom} }

@String { perscomm        = {IEEE Personal Commun. Magazine} }

@String { pimrc           = {Proc., IEEE PIMRC} }

@String { procieee        = {Proceedings of the IEEE} }

@String { sigmag          = {IEEE Signal Processing Magazine} }

@String { sigmetrics      = {Proc., ACM SIGMETRICS} }

@String { spaswin         = {Workshop on Spatial Stochastic Models for Wireless Networks (SPASWIN)} }

@String { transant        = {IEEE Trans. on Antennas and Propagation} }

@String { transcomm       = {IEEE Trans. on Commun.} }

@String { transcontrol    = {IEEE Trans. on Automatic Control} }

@String { transit         = {IEEE Trans. on Info. Theory} }

@String { transmobile     = {IEEE Trans. Mobile Computing} }

@String { transnet        = {IEEE/ACM Trans. on Networking} }

@String { transsig        = {IEEE Trans. on Signal Processing} }

@String { transsmartgrid  = {IEEE Trans. Smart Grid} }

@String { transvt         = {IEEE Trans. on Veh. Technology} }

@String { transwireless   = {IEEE Trans. on Wireless Commun.} }

@String { vehicularmag    = {IEEE Vehicular Technology Magazine} }

@String { vtc             = {Proc., IEEE Veh. Technology Conf. (VTC)} }

@String { wcnc            = {Proc., IEEE Wireless Commun. and Networking Conf. (WCNC)} }

@String { wiopt           = {Proc., Modeling and Optimization in Mobile, Ad Hoc and Wireless Networks} }

@String { wirelessletters = {IEEE Wireless Commun. Letters} }

@String { wirelessmag     = {IEEE Wireless Commun.} }




